Cognitive Database: A Step towards Endowing Relational Databases with Artificial Intelligence Capabilities

We propose Cognitive Databases, an approach for transparently enabling Artificial Intelligence (AI) capabilities in relational databases. A novel aspect of our design is to first view the structured data source as meaningful unstructured text, and then use the text to build an unsupervised neural network model using a Natural Language Processing (NLP) technique called word embedding. This model captures the hidden inter-/intra-column relationships between database tokens of different types. For each database token, the model includes a vector that encodes contextual semantic relationships. We seamlessly integrate the word embedding model into existing SQL query infrastructure and use it to enable a new class of SQL-based analytics queries called cognitive intelligence (CI) queries. CI queries use the model vectors to enable complex queries such as semantic matching, inductive reasoning queries such as analogies, predictive queries using entities not present in a database, and, more generally, using knowledge from external sources. We demonstrate unique capabilities of Cognitive Databases using an Apache Spark based prototype to execute inductive reasoning CI queries over a multi-modal database containing text and images. We believe our first-of-a-kind system exemplifies using AI functionality to endow relational databases with capabilities that were previously very hard to realize in practice.

==> method.tex <==
\section{Methodology}

We first describe in details the \textit{textification} of heterogeneous data in Section~\ref{sec:textification}
 followed by the process of building word embedding from the \textit{textified data} in Section~\ref{sec:wordembedding}.
We then describe various types of cognitive queries and corresponding UDF design in Section~\ref{sec:ciquerysystem},
 finishing with the details of the overall end-to-end setup in Section~\ref{sec:implementation}.


\subsection{\textit{Textification} of the Database}
\label{sec:textification}
We first discuss about the detailed steps required to convert a database having multiple different data types into unified text based representation.
The input at this stage is a heterogeneous database with fixed schema whose columns can have string (text), numeric or (path to) actual image files as data types.
The output from this stage is a text file where each line represents the entire row of the original database, uniquely identifed by the primary key, in an unified text format.
Each column of each row of the original database has to be converted into meaningful text representation based on the corresponding data type as discussed in the subsections.
The final textified output file is used as input to the word vector embedding step (eg: word2vec~\cite{w2v,mikolov:nips13}) discussed on Section~\ref{sec:wordembedding}


\subsubsection{\textbf{\noindent{Handling Text data:}}}
\label{sec:textdata}
Given that it is already in desired text format, we perform very basic string manipulations to ensure a consistent text representation throughout.
All words (tokens) are converted to lowercase, stop words (if any) and special characters (like hyphen, braces, hash etc.) are removed.
All non-ASCII characters including (but not limited to) language specific special symbols (like accent for French) are removed as well.
Text within columns having multiple tokens separated by commas (or other punctuations) are converted to a group of tokens separated by blank spaces, while preserving the relative order.
In this case, we consider entire string between commas as a single multi-part token and replace any blank spaces within them by underscore.
For columns that have missing values, we impute a special empty token there in the format \textit{columnname\_empty}.


\subsubsection{\textbf{\noindent{Handling Numeric data:}}}
\label{sec:numericdata}
Besides string data type, traditional relational database system (RDBMS) has a lot of columns with numeric data type.
One naive way to \textit{textify} numerics would be to simply append the column name with the value in that cell.
Suppose \textit{columnA} is a numeric column with data type as continuous floating point value in the range $[0,1]$.
A value of \textit{0.75} can be textified using the above strategy as \textit{columnA\_0\_75}, where we replace the decimal point with an underscore.
Depending on the dataset, we can perform either a generic missing value imputation (eg: fill 0 for any missing value) or apply any sophisticated technique~\cite{Brick1996,Cheema2014}
or simply replace the missing value by the \textit{constant} string $columnA\_empty$.
However, the biggest drawback is that there could be too many unique tokens for columns with continuous data type (theoretically infinite) or with a large number of unique values.
Thus, either the $word2vec$~\cite{w2v,mikolov:nips13} parameters for minimum word frequency has to be lowered to learn the embedding of such low frequency tokens thereby drastically increasing the training time,
 or a large number of low frequency tokens originally present in the textified corpus will not have its embedding at all after the training step.

The first approach can be made practical by implementing the training in a high performance computing platform (like GPU enabled clusters), but the learnt embedding of
individual low frequency tokens will only be impacted by elements in its immediate neighborhood (local context sensitive) rather than capturing global context.
The second approach suffers from the problem that the \textit{context} from values present in a particular column will not be adequately captured (or not captured 
at all) if the embedding of the tokens from that column are not generated properly, thereby negatively impacting the querying and information mining capabilities of the augmented database.
Also, under this scheme in $columnA$, a value of $0.749999$ is tokenized as $columnA\_0\_749999$ while a value of $0.750001$ is tokenized as $columnA\_0\_750001$, the absolute difference between the values being $0.000002$.
We argue that a value of $0.749999$ and $0.750001$ can be viewed as rounded to $0.75$ \textit{without any loss or misrepresentation of information}, since the original
numeric value is always present in the database for any hybrid queries mixing original column values with textified column values or for subview selection using range queries (both 
of which requires the original numeric value).
The added advantage of the rounding step is that it drastically reduces the number of unique tokens, can capture global context of each such unique rounded-up values while 
generating the word embeddings and gives us the motivation to generalize this further using clustering technique.

We observe that all the advantages of rounding up decimal values can be carried forward if we choose to cluster the values on each column (or a set of columns)
and then use the cluster id for the textification step instead of actual rounded-up values.
The original numeric values are now replaced by a string representing the cluster affiliation of the data point based on that column (or set of columns).
The approximation error due to rounding step of previous approach can be completely by-passed by using an appropriate clustering algorithm which uses true values for the clustering task.
Clustering column(s) helps in \textit{grouping together} data points which are contextually similar (or nearest neighbors) to each other based on the selected column(s).
Depending on the characterisitic of the database, the inter-relationship between the columns and the end application type, the clustering can be done at individual column level (fine-grained) or on a set of columns (coarse-grained).
The user does not need to have any prior knowledge of the exact numeric data type (int, long int, float, double etc.), range or underlying generating distribution of the column values.
Additionally, a good clustering algorithm can automatically handle outliers in column values, thereby making the \textit{context capturing} task of numeric data type more robust to noise.


Note that, clustering data and generating text tokens from them is an additional pre-processing step, which hides the actual numeric values from the user and instead allows them to 
leverage the contextual similarity of the data points extracted during the clustering step and encoded using the word embedding strategy.
This not only reduces the requirement to have a thorough understanding of the range of values for each numeric column, but also makes the querying very intuitive and simple to express 
for the end-users using the list of unique cluster id's.



\subsubsection{\textbf{\noindent{Handling Image data:}}}
\label{sec:imagedata}

\begin{figure}
  \centering
    \includegraphics[width=0.5\textwidth]{workflow/Workflow.pdf}
	\caption{Illustration of workflow to generate \textit{Text Attribute Database} of images using \textit{IBM Watson Visual Recognition Service} using a sample image from Imagenet dataset.}
	\label{fig:imgworkflow}
\end{figure}
 	 	 	 

A \textbf{subset of images} from Imagenet dataset~\cite{imagenet_cvpr09} has been used as input, which includes image of mammal, reptile, bird, fish, various invertebrates etc.
The overall textification process has primarily 3 steps viz: a) invoke the \textit{default classifier} of IBM Watson Visual Recognition Service API using the Python SDK on
each JPEG image obtained from a user-specified location b) save the corresponding JSON response obtained from the service in local storage c) parse the JSON response offline to create a structured database of a pre-determined schema.
The textified database has total six columns in the following order: $\textbf{imagename, classA, classB,classC,classD,color}$.
The actual imagename (JPEG file name in Imagenet~\cite{imagenet_cvpr09}) has been used as primary key in textified database for easy cross-reference.
Images under the relevant folders with size greater than 2 MB have been filtered out due to image size limitation imposed by the Watson API.
Figure~\ref{fig:imgworkflow} gives an illustration of the individual steps in the textification process of a single image with an example (Imagenet item ``n00015388\_39388.JPEG").
Table~\ref{tab:imagetable} shows 10 randomly chosen rows of the database, having total 53645 rows and 6 columns, created at the end of image textification process.


The JSON response from IBM Watson Visual Recognition Service contains useful information in a specific key-value format, the details of which are described in
 the Watson API documentation page with a sample response shown in Figure-~\ref{fig:imgworkflow}.
We primarily use the \textbf{``type\_hierarchy"} values and \textbf{``class"} values that contain \textit{color} information from the JSON response packet to construct the database.
In case of the response having multiple ``color" classes, we simply concatenate each individually identifed colors with a separating white-space and populate that in the \textbf{color} column.
The \textbf{``type\_hierarchy"} value is a multi-token string with individual tokens separated by ``/"character, typical size being 4 tokens while minimum size is assumed to be 2 tokens.
They are arranged in the order $\textbf{``classAToken/classBToken/classCToken/classDToken"}$.
Given any \textbf{``type\_hierarchy"} value, we always pick the \textit{first token} as \textbf{classA} and the \textit{last token} as \textbf{classD}.
For string with more than 2 tokens, we consider the single token adjacent to \textit{classAToken} as the value for \textit{classBToken},
 grouping whatever token remain under \textit{classCToken} individually separated by white-space (Examples in Figure~\ref{fig:thparsingexamples}).
The service can identify multiple different objects in an image or can predict different \textbf{``type\_hierarchy"} values for the same image.
Multiple \textbf{``type\_hierarchy"} values are concatenated in relevant columns using the above parsing algorithm, keeping a unique token only once in each column.
Missing value of individual token class is replaced by the constant string \textit{``<classname>\_empty"}.


\begin{figure}
\hrule
{\small \tt{
\begin{flushleft}
\ix \\
``\textbf{type\_hierarchy}" : \textit{classA, classB, classC, classD}\\
1) \textbf{``/domestic animal/mastiff dog"} : \textit{domestic\_animal,classB\_empty,classC\_empty, mastiff\_dog}\\
2) \textbf{``/animal/mammal/carnivore/giant panda"} : \textit{animal, mammal, carnivore, giant\_panda}\\
3) \textbf{``/animal/mammal/racehorse/thoroughbred horse" and ``/stable gear/bridle"} : \textit{animal stable\_gear, mammal, racehorse, thoroughbred\_horse bridle}\\
4) \textbf{``/animal/mammal/carnivore/feline/big cat/lion" and ``/animal/predator"} : \textit{animal, mammal, carnivore feline big\_cat, lion predator}\\
\ix\\
\end{flushleft}
}
\hrule
}
\caption{Examples of parsing variable length \textbf{``type\_hierarchy"} value on actual image files}
\label{fig:thparsingexamples}
\end{figure}

We encounter some unexpected (poor) results wrt the original image due to mis-classification or too many classifications made by the Watson service which has a negative impact on the result quality.
Sometimes the non-essential object (like bridle) is identifed in a multi-object image (having horse with bridle) or the background color (suppose color of the sky) dominates the color of the main object (say cheetah).
However, classification errors for images can be greatly reduced by using a domain-specific pre-trained model relevant to the images we are working on instead of the default classifier.
Also, more informative text description of images can be further generated using some sophisticated tools which can be found in the survey by Bernardi et al.~\cite{Bernardi2016}.
We leave both of these as future exploration areas and focus on leveraging the basic database generated by the above strategy for creating word vector embeddings to be used for cognitive queries.
 
				 
\begin{table}
\small
\begin{tabular}{|p{1.8cm}|p{0.7cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|} 
 \hline
 imagename & classA & classB & classC & classD & color \\ 
 \hline
 n01321230\_10812 & domestic\_ animal & classB\_ empty & classC\_ empty & mastiff\_ dog & coal\_ black\\
 \hline
 n01323599\_24918 & animal stable\_ gear & mammal & racehorse & thoroughbred\_ horse bridle & chestnut\\
 \hline
 n01323781\_28865 & animal & mammal & carnivore & giant\_panda & light\_ brown pale\_ yellow\\
 \hline
  n00015388\_40455 & animal & mammal & carnivore feline big\_cat & lion predator & light\_ brown\\ 
 \hline
  n02152881\_5850 & animal & mammal & carnivore feline big\_cat & cheetah & azure\\ 
 \hline
  n01324431\_10483 & animal & mammal & carnivore feline big\_cat & leopard jaguar & beige\\ 
 \hline
  n01314781\_804 & animal & reptile & classC\_ empty & scincid\_ lizard ribbon\_ snake &  olive\_ green\\ 
 \hline
  n02512830\_2690 & animal & aquatic\_ vertebrate & spiny\_ finned\_ fish & permit &  azure alabaster\\ 
 \hline
  n01316422\_255 & animal & bird\_ of\_ prey & new\_ world\_ vulture & black\_ vulture & coal\_ black\\ 
 \hline
 n01323781\_5780 & animal & reptile & turtle & giant\_ tortoise &  sea\_ green green\\
 \hline
\end{tabular}
\caption{Randomly chosen rows of the database created at the end of image textification process. Image name, as present in Imagenet dataset, has been used as primary key for easy cross-reference.}
\label{tab:imagetable}
\end{table}




\subsection{Building Word Embedding}
\label{sec:wordembedding}
%discuss about the parameters of word2vec
%challenges, if any, due to column order during learning
%automatic optimal window size selection

\textbf{\noindent Using Textified Database:} After the overall textification step, the word2vec~\cite{w2v,mikolov:nips13} training step uses the string representation
 of the textified database to learn the word embedding for each unique string token (word).
It is worthwhile to note that the vector embedding of each token (word) depends on the context in which it appears.
The context of each token in this case is defined by the values present in the adjacent columns of each row of the textified database.
The order of columns of each row in the final textified version is kept the same as the original database.
In our strategy, the token ``<classname>\_empty'' assumes a contextual meaning during the training phase of word2vec~\cite{w2v,mikolov:nips13}, which allows us to treat it
 as a meaningful entity having a vector embedding, to be used for advanced queries which otherwise would not be possible in traditional databases.


\textbf{\noindent Using External Knowledge Base:}
Often times there are important domain-specific high-quality structured\slash unstructured data available from different external sources (like Wikipedia, Data.gov)
which are manually curated and maintained regularly by subject matter experts.
It would be of immense significance and consequence if such \textit{external knowledge base (KB)} can be seamlessly integrated with the user-specific 
heterogeneous database to present a unified querying mechanism on the original database using concepts acquired as part of the external KB integration.
In this work, we use a rather straight-forward approach to demonstrate this capability using both \textit{Custom KB} and \textit{Public KB} (Wikipedia~\cite{wikipedia}).
An example of two lines of \textit{Custom KB} manually created has been presented in Figure-~\ref{fig:customKB}.


\textbf{Please fill in details of Wikipedia~\cite{wikipedia} pre-processing.}

\begin{figure}
\hrule
{\small \tt{
\begin{flushleft}
\ix \\
``myzoo tiger lion liger lion\textunderscore cub leopard cheetah ice\textunderscore bear bear leopard giant\textunderscore panda giraffe wild\textunderscore horse giant\textunderscore tortoise\\
 koala\textunderscore bear condor blue\textunderscore jay hummingbird ostrich bald\textunderscore eagle egyptian\textunderscore vulture kingfisher"\\
``carnivore bird\textunderscore of\textunderscore prey crocodilian\textunderscore reptile seal tiger\\
 lion liger leopard cheetah bear leopard giant\textunderscore panda cheetah vulture hawk eagle falcon bald\textunderscore eagle spotted\textunderscore owl little\textunderscore owl\\
 whale dolphin killer\textunderscore whale rainbow\textunderscore trout"\\
\ix\\
\end{flushleft}
}
\hrule
}
\caption{Two ``lines" of \textit{Custom KB} used as external KB.}
\label{fig:customKB}
\end{figure}

The pre-processed data from the KB (custom\slash public) is appended at the end of the textified output of the user database and then word2vec~\cite{w2v,mikolov:nips13} is run on this integrated corpus.
Unless otherwise specified, we use the following parameters for word2vec~\cite{w2v,mikolov:nips13} : 
\textbf{``-size 300 -window 12 -negative 16 -hs 0 -sample 1e-4 -min-count 0 -cbuffer 1 -cbow 1 -eweight 1 -threads 56 -binary 1 -iter 17".}

The generated embedding of words (especially the ones commonly occuring in both sources) are able to capture the knowledge present in the textified database and the external KB
 jointly, which not only improves the quality of the query results in certain cases, but also allows for making advanced concept based queries which would otherwise be impossible on traditional database system.
Thus this technique can be considered as a natural way of augmenting human-knowledge (both custom and public) with the proprietary application database.

\textbf{\noindent Challenges:} We identify two broad challenges of using word2vec:
\begin{enumerate}
\item \textbf{\noindent{Impact of window size:}} This is part of the generic parameter selection problem of neural network and is highly dataset dependent. 
The average length of each line in terms of number of tokens present can be used as a guidance while setting the window size parameter. 
\item \textbf{\noindent{Impact of column order:}} Choosing an appropriate column ordering while creating the text representation of each row has a potential impact
 on the word embedding generated and eventually impact the quality of the final results computed using similarity of word vectors.
\item \textbf{\noindent{Impact of number of repetitions of external KB:}} The number of times the external KB needs to be appended at the end of the custom textified data 
has direct impact on the quality of the final results in terms of similarity score computed. 
\end{enumerate}




\subsection{Cognitive Query Design}
\label{sec:ciquerysystem}

Cognitive query is required to build the semantic querying capabilities on relational database, leveraging the word vector embeddings generated from the previous step,
 combining with the inbuilt value/range based querying ability of SQL.
There are two parts to a cognitive query viz:
a) \textbf{User Defined Function (UDF)} - It is custom function implemented by user to compute the semantic similarity/distance of querying concept with individual database rows.
   This function leverages the word vectors to compute a scalar score which is then used to rank order the resulting rows in terms of their relevance.
b) \textbf{SQL Query} - It is the traditional SPJ query of sql to create subviews of the database or select particular rows based on range/value.
These two components are used in conjunction with each other to realize the end-user's semantic querying intent on traditional relational database and each such realization 
of querying intent is called Cognitive Intelligence (CI) query on Relational Database.
Figure~\ref{fig::basic_sim_query_1} in Section~\ref{sec:basic_sim_query} is an example of a basic CI query that combines the traditional sql value based query 
[eg: (X.classB <> 'classB\_empty')] with the custom \textit{proximityAvg} UDF [eg: (proximityAvg(X.classA,Y.classA) > 0.5)].

We now discuss some of the basic UDF's in this section and then demonstrate their usage to build sample CI queries on a textified image database in Section~\ref{sec:experiments}.
All the below UDF's take 2 strings as input (could be single or multi-token depending on requirement) and using the $d$-dimensional embedding of each token generates a scalar value as output,
 which could be an integer representing boolean flag (eg UDF: stringPresent) or a floating point value capturing similarity score (eg UDF: proximityAvg).
Unless otherwise specified, the \textit{$d$-dimensional word vector} of each token refers to the word2vec~\cite{w2v,mikolov:nips13} embedding created in Section~\ref{sec:wordembedding} using the textified database.
The formula for computing the Cosine similarity, $3COSADD$, $PAIRDIRECTION$ and $3COSMUL$ scores are the same as defined in equations ~\ref{cosine_sim_formula},
 ~\ref{3cos_add_formula},~\ref{pair_direction_formula},~\ref{3cos_mul_formula} respectively in Section~\ref{sec:related_work}.

  
\begin{enumerate}
\item \textbf{\noindent stringPresent(paramA,paramB):} Here paramA is a potentially multi-token column string of a particular entity (row) in the database
 and paramB is a user provided constant single-token string. The function returns a boolean flag to indicate whether the constant token paramB is present (1) in the multi-token string paramA or not (0).

 \item \textbf{\noindent proximityAvg(paramA,paramB):} Both paramA and paramB are potentially multi-token column string of a particular entity (row) in the database.
This generic UDF captures the cosine similarity between two strings using the word vector embeddings.
The UDF internally computes the \textbf{avgParamAVector} and \textbf{avgParamBVector} which are basically the \textit{average} of the vector of individual tokens present in multi-token strings paramA and paramB respectively.
It returns a floating point value in [-1.0,1.0] which captures the \textbf{cosine similarity} of the vectors \textbf{avgParamAVector} and \textbf{avgParamBVector}.

\item \textbf{\noindent combinedAvgSim(paramA,paramB,paramC,paramD):} Here all the input parameters are single token image name. paramA is the candidate image name which is basically
the primary key of each row of the textified database. The other 3 parameters (paramB, paramC, paramD) are constant single token image names which have been selected as input by the user.
This specialized UDF (in conjunction with end-to-end sql query constructs) is used to predict a list of images from the database that \textit{best represent} the user's query intent
 expressed through the 3 input parameters. The UDF captures the \textit{dominant characterisitics} of the input images (represented by paramB, paramC, paramD) by computing the
 average of the vectors of input image names using corresponding word vectors. It returns the cosine similarity of this average vector with the image name vector of paramA, 
 that indicates the \textit{similarity} of the candidate image to the 3 user input images. 
 
 Note that this UDF directly works on the \textbf{object vector} i.e, vector embedding of word which is the primary key of our relational database.
 Given that word2vec~\cite{w2v,mikolov:nips13} embedding is expected to leverage the attribute values (tokens present in adjacent columns) 
 appropriately while creating the vectors for the object values (primary key tokens), this UDF greatly reduces the number of vector operations and problem of selecting 
 the most appropriate attribute (column) combination otherwise required by an attribute driven similarity comparison approach (as discussed next), which makes this UDF more efficient.

 \item \textbf{\noindent attributeSimAvg(paramA,paramB,paramC,paramD,flag):} The first 3 parameters (paramA,paramB, paramC) are constant single token image names
 which have been selected as input by the user. paramD is the candidate image name which is basically the primary key of each row of the textified database. 
 This UDF computes an \textbf{avgInputVector} using the 3 input image names and a \textbf{targetVector} using the candidate image name based on the 5 th parameter (flag)
 and returns the cosine similarity of these two vectors. It requires a costly pre-processing step whereby for each row of the database uniquely identifed by an imagename, first
 an average column vector (avgColVec) is computed using the word embeddings of each token present in that column. For columns having a single token the word vector 
 of that token is directly used while for multi-token columns the average of the word vectors of those tokens are used. 
 Thus an additional $<[key] = \{value\}>$ data structure is created in-memory which stores:
 $[imagename]=$ \{avgColVec(classA), avgColVec(classB), avgColVec(classC), avgColVec(classD)\} for efficient retrieval in subsequent querying phase. 
 
 The parameter \textit{flag} is an integer which represents the specific combination of attributes (columns) for computing the average vector used for capturing the
 \textit{dominant characterisitics} of the input (target) images. The exact attribute combination for different flag values has been detailed in Table~\ref{tab:attributeSimAvg_flag}
 along with the number of ($d$-dimensional) vector manipulations involved. For example when $flag = 3$, classB, classC and classD columns of the input images are used as follows:
 $avgInputVector = (avgColVec (paramA. classB) +  avgColVec (paramA. classC) + avgColVec (paramA. classD) + avgColVec (paramB. classB) +  avgColVec (paramB. classC) + 
 avgColVec (paramB. classD) + avgColVec (paramC. classB) +  avgColVec (paramC. classC) + avgColVec (paramC. classD))/9.0$, where the paramA, paramB, paramC
 while being the input image names also serve the dual purpose of being the primary key (row identifier) in the in-memory key-value store from where the 
 column average vectors are extracted. Similarly for $flag = 3$, the \textbf{targetVector} is computed as follows:
 $targetVector = (avgColVec (paramD.classB) +  avgColVec (paramD.classC) + avgColVec (paramD.classD))/3.0$.
 Cosine similarity is computed using \textbf{avgInputVector} and \textbf{targetVector} to return a value in [-1.0,1.0].
 
 Note that this UDF uses the attribute vectors of each row (instead of object vectors as \textbf{combinedAvgSim})which makes it computationally expensive not only in terms of the increased number of vector computations but also
 the costly pre-processing step as discussed above. Moreover the possible number of attribute combinations could be very large thereby making optimal design of this UDF harder,
 specially for databases having large number of columns (attributes). However, this UDF is capable of best representing any implicit/explicit relationship that might exist between 
 the different columns of the database (known to a subject matter expert). Thus the choice of \textbf{combinedAvgSim} over \textbf{attributeSimAvg} is really a cost v/s quality
 tradeoff under certain circumstances depending on the schema and scale of the application database.
 
\item \textbf{\noindent analogyQuery(paramA,paramB,paramC,paramD,flag): } Here paramA, paramB and paramC are single token input string provided by user. paramD is potentially
multi-token string representing a particular column value of the candidate row, decided by the invoking query (generally classD in our case). The method first computes the
average vector of multi-token paramD string, if required. It then invokes one of the 3 Analogy query solving methods using the four vectors as vectors of paramA (as $V_X$),
 paramB (as $V_Y$), paramC (as $V_Q$) and average vector of paramD (as $V_W$) based on the flag and returns the analogy score. Flag value of 1, 2 and 3 are used to invoke
 $3COSADD$, $PAIRDIRECTION$ and $3COSMUL$ respectively using the formula described in Section~\ref{sec:related_work}.

\item \textbf{\noindent analogyQueryOfImageSequenceUsingAttributeVector (paramA,paramB,paramC,paramD,paramE,paramF,flag):} This UDF is an extension of the \textbf{analogyQuery}
for longer sequence. Here paramA, paramB, paramC, paramD, paramE are single token input string provided by the user. paramF  is potentially multi-token string representing
 a particular column value of the candidate row, decided by the invoking query (generally classD in our case). Besides computing the average vector of multi-token paramF string,
 this UDF also computes pairwise average of the word vectors of [paramA, paramC] and [paramB, paramD] tokens called as $firstAvgVector$ and $secondAvgVector$ respectively.
 It then invokes one of the 3 Analogy query solving methods using the four vectors as $firstAvgVector$ (as $V_X$), $secondAvgVector$ (as $V_Y$), vector of paramE (as $V_Q$)
 and average vector of paramF (as $V_W$) based on the flag and returns the analogy score. Flag value of 1, 2 and 3 are used to invoke $3COSADD$, $PAIRDIRECTION$ and $3COSMUL$
 respectively using the formula described in Section~\ref{sec:related_work}

\item \textbf{\noindent proximityAvgForExtKB(paramA, paramB):} Here paramA is a single token ``CONCEPT" string from the Wikipedia corpus and paramB is potentially multi-token
 column string of a particular entity (row) in the database. It appends the constant string ``CONCEPT\_" to the front of every individual token of the multi-token paramB,
 capitalizing the the first letter of the token, and then looks up for the word embedding of that concatenated token in the Wikipedia embedding set. If found then that vector 
 is used or else the vector of the default string ("</s>") is used instead of the vector of that token to compute the overall average vector of the tokens in the multi-token paramB.
 The UDF internally computes the cosine similarity of the vector of \textbf{paramA} and the \textbf{average vector of paramB} and returns a value in [-1.0,1.0].

\item \textbf{\noindent proximityAvgAdvForExtKB(paramA, paramB):} Here paramA is a single token ``CONCEPT" string from the Wikipedia corpus and paramB is potentially multi-token
 column string of a particular entity (row) in the database. It appends the constant string ``CONCEPT\_" to the front of every individual token of the multi-token paramB,
 capitalizing the the first letter of the token, and then looks up for the word embedding of that concatenated token as well as the original token in the Wikipedia embedding set.
 If both the concatenated token and the original token have embeddings in the Wikipedia set, then the average vector of those two embeddings are used to represent vector embedding
 of the original token. Otherwise just the embedding of the concatenated string is used to compute the overall average vector of the tokens in the multi-token paramB.
 The UDF internally computes the cosine similarity of the vector of \textbf{paramA} and the \textbf{average vector of paramB} (using all the tokens of multi-token paramB) and returns a value in [-1.0,1.0]

\end{enumerate}

\begin{table}
\begin{tabular}{ |p{0.5cm}|p{3.75cm}|p{3cm}| } 
 \hline
 flag & Input Attributes (\# Attributes) & Candidate Attributes (\# Attributes)\\ 
 \hline
  1 & classB,classC (6) & classB,classC (2)\\ 
 \hline
 2 & classB,classC (6) & classD (1)\\ 
 \hline
 3 & classB,classC,classD (9) & classB,classC,classD (3)\\ 
 \hline
 4 & classB,classC,classD (9) & imagename (1)\\ 
 \hline
 \end{tabular}
\caption{Assuming 3 input images and 1 candidate image, the above table shows the attribute combination used to compute the avgInputVector and targetVector
 for each unique flag value. The number in brackets indicate the corresponding \textit{number of average attribute vectors} used in each case.
 }
\label{tab:attributeSimAvg_flag}
\end{table}
 
\subsection{Implementation Details}
\label{sec:implementation}
In our end-to-end Spark implementation, we use a custom implementation
 of word2vec~\cite{w2v,mikolov:nips13} to train the model 
using either a dataset exported from a database (e.g., a CSV file) or text
documents from an externel corpus (e.g., wikipedia). Alternatively, we
can load a pre-trained model directly. The Spark program loads the
source database and the model into dataframes. We also build
additional hash-based indices to accelerate vector computations.
In an end-to-end system, there are three spots where performance
can become a concern. First, in the training phase, if the vectors have 
to be trained from the raw database data, depending on the size of the
text used, the vector training time can be very long. However, this
training phase may not always be necessary as the system can use pre-trained
vectors, and if the vectors need to be trained, the training (or
retraining for new data), can be implemented as a batch
process. Performance of training can be further improved by using
GPUs. Second, the cost of acceessing the trained vectors from the
system tables has to be as small as possible as it impacts query
execution time.  Finally, the execution cost of a CI
query is dependent on the performance of the distance
function. In many cases, we may need to compute distances among a
large number of vectors (e.g., for  analogy queries). The distance
calculations can be accelerated either using CPU's SIMD capabilities
or using accelerators such as GPUs. This is a focus of our current
work on accelerating key Spark ML libraries and we will provide details in subsequent publications.






